WiSoSuper: Benchmarking Super-Resolution Methods on Wind and Solar Data

The transition to green energy grids depends on detailed wind and solar forecasts to optimize the siting and scheduling of renewable energy generation. Operational forecasts from numerical weather prediction models, however, only have a spatial resolution of 10 to 20-km, which leads to sub-optimal usage and development of renewable energy farms. Weather scientists have been developing super-resolution methods to increase the resolution, but often rely on simple interpolation techniques or computationally expensive differential equation-based models. Recently, machine learning-based models, specifically the physics-informed resolution-enhancing generative adversarial network (PhIREGAN), have outperformed traditional downscaling methods. We provide a thorough and extensible benchmark of leading deep learning-based super-resolution techniques, including the enhanced super-resolution generative adversarial network (ESRGAN) and an enhanced deep super-resolution (EDSR) network, on wind and solar data. We accompany the benchmark with a novel public, processed, and machine learning-ready dataset for benchmarking super-resolution methods on wind and solar data.

==> NeurIPS2020/lutjens_utils.tex <==

%\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{graphicx} % more modern
%\usepackage{epsfig} % for postscript graphics files
\usepackage{amsfonts}
\usepackage{amsmath,soul}
\usepackage{amssymb}
\usepackage[capitalize]{cleveref} %cref
%\crefformat{equation}{(#2#1#3)}%
%\Crefformat{equation}{Equations~(#2#1#3)}
%\Crefname{equation}{Equation}{}

\usepackage{dsfont} % mathds
\usepackage[font=small,skip=0pt]{subcaption} %subfigure
\usepackage{balance}
\usepackage[font=small]{caption}
\usepackage{bm} % bold italic vectors
\usepackage{wrapfig}
\usepackage{float} % To place figure on top right as float

% Define special colors
\usepackage{color}
%\usepackage[svgnames]{xcolor} \definecolor{DarkGreen}{rgb}{0,0.5,0}
%\definecolor{DarkRed}{rgb}{0.75,0,0}

\def\name/{\textit{PCE-PINNs}}

% Define author comments
\usepackage[authormarkuptext=name,addedmarkup=bf,authormarkupposition=left]{changes}
%\usepackage[final]{changes} %Use this to hide all comments.
\definechangesauthor[name={J.~H.}, color={blue}]{jh}
\definechangesauthor[name={M.~E.}, color={red}]{me}
\definechangesauthor[name={B.~L.}, color={green}]{bl}
\setlength {\marginparwidth }{2cm}
\newcommand{\XX}[1]{\added[id=jh,remark={}]{#1}}
\newcommand{\meXX}[1]{\added[id=me,remark={}]{#1}}
\newcommand{\blXX}[1]{\added[id=bl,remark={}]{#1}}
\newcommand{\jsec}[1]{\marginpar{\fcolorbox{yellow}{yellow}{\parbox{0.7in}{\raggedright
        \color{blue} \tiny #1 }}}}
\newcommand{\hsec}[1]{\marginpar{\fcolorbox{yellow}{yellow}{\parbox{0.7in}{\raggedright
        \color{green} \tiny #1 }}}}
\newcommand{\jhmargin}[2]{{\color{orange}#1}\marginpar{\color{red}\tiny\raggedright
    \bf [JH] #2}}
\newcommand{\blmargin}[2]{{\color{green}#1}\marginpar{\color{green}\tiny\raggedright
    \bf [BL] #2}}

% tikz
\usepackage{tikz,mathtools}
\crefformat{equation}{(#2#1#3)}
\Crefformat{equation}{Equation~(#2#1#3)}
\Crefname{equation}{Equation}{Equations}
\newcommand{\inputTikZ}[2]{\scalebox{#1}{\input{#2}}}
\usetikzlibrary{shapes,positioning,automata,arrows,fit,backgrounds,calc}
\tikzstyle{block} = [draw, fill=blue!20, rectangle,minimum height=1em,
minimum width=2em] \tikzstyle{sum} = [draw, fill=blue!20, circle, node
distance=1cm] \tikzstyle{input} = [coordinate] \tikzstyle{output} =
[coordinate] \tikzstyle{pinstyle} = [pin edge={to-,thin,black}]
\usetikzlibrary{trees} \usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.markings}
\definecolor{darkgreen}{rgb}{0,0.5,0}
\definecolor{darkred}{rgb}{220,20,60}

% Define argmin argmax
%\DeclareMathOperator*{\argmin}{\arg\!\min}
%\DeclareMathOperator*{\argmax}{\arg\!\max}

% Single line comment
\newcommand{\cmmnt}[1]{\ignorespaces}

% Define commands for itemized lists
\newcommand{\bit}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}

